Infinitary Axiomatization of the Equational Theory of Context-Free Languages

We give a natural complete infinitary axiomatization of the equational theory of the context-free languages, answering a question of Lei{\ss} (1992).

==> eptcsdata.tex <==
\providecommand{\firstpage}{44}
\providecommand{\publicationstatus}{D. Baelde and A. Carayol (Eds.): Fixed Points\\
in Computer Science 2013 (FICS 2013)\\
EPTCS 126, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.126.4}{10.4204/EPTCS.126.4}}

